Controllable tunnelling of single flux-quanta mediated by quantum phase-slip in disordered superconducting loops

Quantum phase-slip (QPS) is the exact dual to the well-known Josephson effect. Although there are numerous proposals for applications of QPS devices, experimental work to develop these remains in the relatively early stages. Significant barriers to exploiting QPS nanowires for useful technologies still exist, such as establishing robust nanowire fabrication methods that allow coupling to low-loss circuits, and demonstrating control over the QPS process with an experimenter-controlled external bias. Here we report experiments which show that both of these barriers have been overcome. We present measurements at 300 mK of NbN coplanar waveguide (CPW) resonators embedded with nanowires fabricated using a neon focused ion-beam. The internal quality factor exceeds $2\times10^{4}$ -- significantly higher than previously reported in comparable experiments. The resonator frequency tunes periodically with an applied magnetic field, revealing tunnelling of the order parameter that always occurs at half-integer values of the applied flux. In contrast to previous studies of single QPS, the order-parameter tunnelling is shown to be adiabatic, demonstrating improved control over energy dissipation in nanowire QPS circuits. Our results highlight a promising pathway towards realising low-loss nanowire-based QPS devices.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
